Modulation Analysis with Higher-Order Spectra

A need to identify modulation of spectral power arises frequently in the analysis of physiological signals. Estimation of power in the relevant bands through filtering and envelope extraction has several limitations: the choice of filter may bias any resulting estimate, while additive Gaussian noise becomes non-Gaussian due to the nonlinearity of envelope computation. The present work considers how spectral decompositions of higher-order cumulants (higher-order spectra, HOS) avoid these limitations, with an emphasis on the use of the trispectrum to identify modulated oscillations. Specifically, it is shown: 1) The trispectrum may be interpreted as a measure of linear dependencies of power across frequencies by viewing it as the cross spectrum of the Wigner-Ville distribution. 2) A particular two-dimensional subdomain of the trispectrum is useful for identifying modulated carriers, recovering essential spectral properties of both the modulating and carrier signals while avoiding the cubic complexity of full trispectrum estimation. A representation of this subdomain, the modulogram, is demonstrated as a tool for identifying and distinguishing different forms of modulation. 3) As a cumulant-derived measure, the modulogram is not biased by additive Gaussian noise. 4) Modulogram phase retains information by which temporal patterns of modulation may be identified. 5) A recently described additive decomposition of HOS (HOSD) further aids identification when applied to the trispectrum. These developments are illustrated with the blind detection of beta bursts in rodent and human local field potential recordings. Finally, the relationship between the present approach and prior techniques of blind identification (BI) through moment maximization, including blind deconvolution and independent component analysis, is considered.

==> mathcolor.ltx <==
%%
%% This is file `mathcolor.ltx',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% mathcolor.dtx  (with options: `code')
%% 
%% The source is maintained by the LaTeX Project team and bug
%% reports for it can be opened at https://latex-project.org/bugs/
%% (but please observe conditions on bug reports sent to that address!)
%% 
%% 
%% File: mathcolor.dtx (C) Copyright 2021-2022
%%% From File: mathcolor.dtx
\def\mathcolorversion{v1.0c}
\def\mathcolordate{2022/07/25}
\ifcsname mathcolor\endcsname \endinput \fi
\ExplSyntaxOn
\seq_new:N \g__mathcolor_seq
\DeclareDocumentCommand \mathcolor { o m m }
  {
    \mode_if_math:F { \non@alpherr {\mathcolor\space} }
    \seq_gpush:No \g__mathcolor_seq \current@color
    \group_insert_after:N \use_none:n
    \IfValueTF {#1} { \color[#1]{#2} } { \color{#2} }
    #3
    \__mathcolor_scan_for_scripts:w
  }
\cs_new_protected:Npn \__mathcolor_scan_for_scripts:w
  {
    \peek_remove_filler:n
      {
        \group_align_safe_begin:
        \token_case_catcode:NnTF \l_peek_token
          {
            \c_math_subscript_token { }
            \c_math_superscript_token { }
          }
          { \__mathcolor_handle_scripts:Nw }
          {
            \token_case_meaning:NnTF \l_peek_token
              {
                \limits   { \limits }
                \nolimits { \nolimits }
                \displaylimits { \displaylimits }
              }
              {
                \group_align_safe_end:                          % case 4
                \__mathcolor_scan_for_scripts:w \use_none:n
              }
              {
                \token_if_eq_meaning:NNTF \l_peek_token '
                  {
                    \__mathcolor_handle_scripts:Nw ^
                    \c_group_begin_token
                      \exp_after:wN \prim@s \use_none:n
                  }
                  {
                    \group_align_safe_end:                      % case 1
                    \reset@color
                    \seq_gpop:NN \g__mathcolor_seq \current@color
                  }
              }
          }
      }
  }
\cs_new_protected:Npn \__mathcolor_handle_scripts:Nw #1
  {
    #1 \c_group_begin_token \c_group_begin_token
    \seq_get:NN \g__mathcolor_seq \current@color
    \set@color
    \group_insert_after:N \c_group_end_token
    \group_insert_after:N \__mathcolor_scan_for_scripts:w
    \peek_remove_filler:n
      {
        \token_if_eq_meaning:NNTF \l_peek_token \c_group_begin_token
          {
            \group_align_safe_end:                              % case 2
            \peek_catcode_remove:NT \c_group_begin_token { }
          }
          {
            \exp_after:wN \group_align_safe_end:                % case 3
              \use_ii_i:nn \c_group_end_token
          }
      }
  }
\ExplSyntaxOff
%%%%%%%%%%%%%%%%
\endinput
%%
%% End of file `mathcolor.ltx'.

